Light Communication for Controlling Industrial Robots

Optical Wireless Communication (OWC) is regarded as an auspicious communication approach that can outperform the existing wireless technology. It utilizes LED lights, whose subtle variation in radiant intensity generate a binary data stream. This is perceived by a photodiode, that converts it to electric signals for further interpretation. This article aims at exploring the use of this emerging technology in order to control wirelessly industrial robots, overcoming the need for wires, especially in environments where radio waves are not working due to environmental factors or not allowed for safety reasons. We performed experiments to ensure the suitability and efficiency of OWC based technology for the aforementioned scope and "in vitro" tests in various Line-of-Sight (LoS) and Non-Line-of-Sight (NLoS) configurations to observe the system throughput and reliability. The technology performance in the "clear LoS" and in the presence of a transparent barrier, were also analyzed.

==> OWC Robots control Final/abstract.tex <==
\chapter{Abstract}
\label{chap:Abstract}

Visible Light Communications is a relatively old technology that lately has sped up his development dramatically. It uses LED lights to generate a binary data stream, whose subtle changes in luminosity intensity are sensed by a photodiode, which converts it to electric signal, ready to be interpreted. This project aims to study the use case of this emerging technology to wirelessly control industrial robots, in order to overcome the needs for wires, especially in environments where radio waves are not working due to environmental factors or not allowed due to safety reasons. Hence, will be done tests in order to ensure if the technology is appropriate for the scope and will be elaborated proposals so that the system can be used in a real-life scenario.

==> abstract.tex <==
\chapter{Abstract}
\label{chap:Abstract}

Visible Light Communications is a relatively old technology that lately has sped up his development dramatically. It uses LED lights to generate a binary data stream, whose subtle changes in luminosity intensity are sensed by a photodiode, which converts it to electric signal, ready to be interpreted. This project aims to study the use case of this emerging technology to wirelessly control industrial robots, in order to overcome the needs for wires, especially in environments where radio waves are not working due to environmental factors or not allowed due to safety reasons. Hence, will be done tests in order to ensure if the technology is appropriate for the scope and will be elaborated proposals so that the system can be used in a real-life scenario.
